Did you miss it? Automatic lung nodule detection combined with gaze information improves radiologists' screening performance

Early diagnosis of lung cancer via computed tomography can significantly reduce the morbidity and mortality rates associated with the pathology. However, search lung nodules is a high complexity task, which affects the success of screening programs. Whilst computer-aided detection systems can be used as second observers, they may bias radiologists and introduce significant time overheads. With this in mind, this study assesses the potential of using gaze information for integrating automatic detection systems in the clinical practice. For that purpose, 4 radiologists were asked to annotate 20 scans from a public dataset while being monitored by an eye tracker device and an automatic lung nodule detection system was developed. Our results show that radiologists follow a similar search routine and tend to have lower fixation periods in regions where finding errors occur. The overall detection sensitivity of the specialists was 0.67$\pm$0.07, whereas the system achieved 0.69. Combining the annotations of one radiologist with the automatic system significantly improves the detection performance to similar levels of two annotators. Likewise, combining the findings of radiologist with the detection algorithm only for low fixation regions still significantly improves the detection sensitivity without increasing the number of false-positives. The combination of the automatic system with the gaze information allows to mitigate possible errors of the radiologist without some of the issues usually associated with automatic detection system.

==> characterization.tex <==
\subsection{Nodule characterization agreement}

Table~\ref{tab:characteristics} shows the percentage of nodules that, for each ordinal characteristic, are outside the the range defined by the average of the LIDC-IDRI annotators $\pm$ the standard deviation. All radiologists have disagreed on at least 2 characteristics, in comparison with the ground-truth, for at least 60\% of the nodules. Also, the nodule characteristic with highest agreement is the texture, and the lowest are sphericity, expected malignancy and subtlety.

\begin{table}[]
    \caption{Percentage of nodules which characterization is outside the range defined by the average of the LIDC-IDRI annotators $\pm$ the standard deviation of the respective abnormality. $n$: number of considered nodules. $\geq \#$: outside on at least $\#$ of the characteristics. \label{tab:characteristics}}
    \centering
    \begin{tabular}{|c|c|c|c|c||c|} \hline
Characteristic&\makecell{Rad 1\\$n=25$}&\makecell{Rad 2\\$n=32$}&\makecell{Rad 3\\$n=29$}&\makecell{Rad 4\\$n=25$}&\makecell{Avg. $\pm$ \\ std }\\\hline
Lobulation&40&31&38&\textbf{16}&31$\pm$9\\\hline
Malignancy&32&\textbf{28}&59&48&41$\pm$12\\\hline
Margin&40&25&66&\textbf{20}&37$\pm$17\\\hline
Sphericity&56&\textbf{44}&52&56&51$\pm$4\\\hline
Spiculation&\textbf{12}&16&38&64&32$\pm$20\\\hline
Subtlety&40&\textbf{31}&69&36&44$\pm$14\\\hline
Texture&12&31&45&\textbf{8}&24$\pm$14\\\hline\hline
All&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&0$\pm$0\\\hline
$\geq 3/4$&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&0$\pm$0\\\hline
$\geq 1/2$&16&\textbf{9}&59&20&26$\pm$19\\\hline
$\geq 1/4$&\textbf{64}&69&93&84&77$\pm$11\\\hline
At least one&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&100$\pm$0\\\hline
    
    \end{tabular}
\end{table}


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> table.tex <==
$\blacksquare$$\square$$\square$$\square$$\square$&0.87&0.4$\pm$0.49&1.9$\pm$2.21&3.6$\pm$2.46\\\hline
$\square$$\blacksquare$$\square$$\square$$\square$&0.8&0.1$\pm$0.3&1.1$\pm$1.58&2.4$\pm$1.91\\\hline
$\square$$\square$$\blacksquare$$\square$$\square$&0.93&0.1$\pm$0.3&0.9$\pm$1.22&2.4$\pm$1.28\\\hline
$\square$$\square$$\square$$\blacksquare$$\square$&0.87&0.1$\pm$0.3&0.8$\pm$1.17&2.2$\pm$1.17\\\hline
$\square$$\square$$\square$$\square$$\blacksquare$&0.8&0.0$\pm$0.0&0.1$\pm$0.3&1.3$\pm$0.78\\
$\square$$\square$$\square$$\square$$\blacksquare$&0.87&0.1$\pm$0.3&0.1$\pm$0.3&1.5$\pm$0.92\\
$\square$$\square$$\square$$\square$$\blacksquare$&0.93&0.2$\pm$0.4&0.1$\pm$0.3&1.7$\pm$0.78\\
$\square$$\square$$\square$$\square$$\blacksquare$&1.0&0.3$\pm$0.46&0.2$\pm$0.4&2.0$\pm$0.89\\\hline
$\blacksquare$$\blacksquare$$\square$$\square$$\square$&0.93&0.5$\pm$0.67&1.9$\pm$1.92&3.8$\pm$2.14\\\hline
$\blacksquare$$\square$$\blacksquare$$\square$$\square$&0.93&0.5$\pm$0.5&1.7$\pm$1.79&3.6$\pm$1.96\\\hline
$\blacksquare$$\square$$\square$$\blacksquare$$\square$&0.93&0.5$\pm$0.5&1.9$\pm$1.76&3.8$\pm$2.04\\\hline
$\blacksquare$$\square$$\square$$\square$$\blacksquare$&1.0&0.4$\pm$0.49&1.5$\pm$1.63&3.4$\pm$1.96\\\hline
$\square$$\blacksquare$$\blacksquare$$\square$$\square$&0.93&0.2$\pm$0.4&1.1$\pm$1.58&2.7$\pm$1.68\\\hline
$\square$$\blacksquare$$\square$$\blacksquare$$\square$&0.87&0.2$\pm$0.4&1.3$\pm$1.49&2.8$\pm$1.54\\\hline
$\square$$\blacksquare$$\square$$\square$$\blacksquare$&0.93&0.1$\pm$0.3&1.0$\pm$1.34&2.5$\pm$1.69\\
$\square$$\blacksquare$$\square$$\square$$\blacksquare$&1.0&0.3$\pm$0.46&1.1$\pm$1.58&2.9$\pm$1.64\\\hline
$\square$$\square$$\blacksquare$$\blacksquare$$\square$&0.93&0.2$\pm$0.4&0.9$\pm$0.94&2.5$\pm$0.92\\\hline
$\square$$\square$$\blacksquare$$\square$$\blacksquare$&1.0&0.1$\pm$0.3&0.6$\pm$0.8&2.2$\pm$1.08\\\hline
$\square$$\square$$\square$$\blacksquare$$\blacksquare$&0.93&0.1$\pm$0.3&0.7$\pm$0.9&2.2$\pm$1.17\\
$\square$$\square$$\square$$\blacksquare$$\blacksquare$&1.0&0.3$\pm$0.46&0.8$\pm$0.98&2.6$\pm$1.02\\\hline
$\blacksquare$$\blacksquare$$\blacksquare$$\square$$\square$&0.93&0.6$\pm$0.66&1.9$\pm$1.92&3.9$\pm$2.02\\\hline
$\blacksquare$$\blacksquare$$\square$$\blacksquare$$\square$&0.93&0.6$\pm$0.66&2.1$\pm$1.92&4.1$\pm$2.12\\\hline
$\blacksquare$$\blacksquare$$\square$$\square$$\blacksquare$&1.0&0.5$\pm$0.67&1.9$\pm$1.92&3.9$\pm$2.21\\\hline
$\blacksquare$$\square$$\blacksquare$$\blacksquare$$\square$&0.93&0.6$\pm$0.49&1.9$\pm$1.76&3.9$\pm$1.92\\\hline
$\blacksquare$$\square$$\blacksquare$$\square$$\blacksquare$&1.0&0.5$\pm$0.5&1.7$\pm$1.79&3.7$\pm$2.0\\\hline
$\blacksquare$$\square$$\square$$\blacksquare$$\blacksquare$&1.0&0.5$\pm$0.5&1.9$\pm$1.76&3.9$\pm$2.07\\\hline
$\square$$\blacksquare$$\blacksquare$$\blacksquare$$\square$&0.93&0.3$\pm$0.46&1.4$\pm$1.69&3.1$\pm$1.58\\\hline
$\square$$\blacksquare$$\blacksquare$$\square$$\blacksquare$&1.0&0.2$\pm$0.4&1.1$\pm$1.58&2.8$\pm$1.72\\\hline
$\square$$\blacksquare$$\square$$\blacksquare$$\blacksquare$&0.93&0.2$\pm$0.4&1.3$\pm$1.49&2.9$\pm$1.64\\
$\square$$\blacksquare$$\square$$\blacksquare$$\blacksquare$&1.0&0.4$\pm$0.49&1.4$\pm$1.69&3.3$\pm$1.55\\\hline
$\square$$\square$$\blacksquare$$\blacksquare$$\blacksquare$&1.0&0.2$\pm$0.4&0.9$\pm$0.94&2.6$\pm$1.02\\\hline
$\blacksquare$$\blacksquare$$\blacksquare$$\blacksquare$$\square$&0.93&0.7$\pm$0.64&2.1$\pm$1.92&4.2$\pm$1.99\\\hline
$\blacksquare$$\blacksquare$$\blacksquare$$\square$$\blacksquare$&1.0&0.6$\pm$0.66&1.9$\pm$1.92&4.0$\pm$2.1\\\hline
$\blacksquare$$\blacksquare$$\square$$\blacksquare$$\blacksquare$&1.0&0.6$\pm$0.66&2.1$\pm$1.92&4.2$\pm$2.18\\\hline
$\blacksquare$$\square$$\blacksquare$$\blacksquare$$\blacksquare$&1.0&0.6$\pm$0.49&1.9$\pm$1.76&4.0$\pm$1.95\\\hline
$\square$$\blacksquare$$\blacksquare$$\blacksquare$$\blacksquare$&1.0&0.3$\pm$0.46&1.4$\pm$1.69&3.2$\pm$1.66\\\hline
$\blacksquare$$\blacksquare$$\blacksquare$$\blacksquare$$\blacksquare$&1.0&0.7$\pm$0.64&2.1$\pm$1.92&4.3$\pm$2.05\\\hline
